Seamless, Correct, and Generic Programming over Serialised Data

In typed functional languages, one can typically only manipulate data in a type-safe manner if it first has been deserialised into an in-memory tree represented as a graph of nodes-as-structs and subterms-as-pointers. We demonstrate how we can use QTT as implemented in \idris{} to define a small universe of serialised datatypes, and provide generic programs allowing users to process values stored contiguously in buffers. Our approach allows implementors to prove the full functional correctness by construction of the IO functions processing the data stored in the buffer.

==> Data/Singleton.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Data.Singleton}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*singleton>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{x}
\end{code}
%</singleton>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaSpace{}\IdrisKeyword{\%unsafe}\KatlaNewline{}
\IdrisFunction{unsafeMkSingleton}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\IdrisPostulate{unsafeMkSingleton}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisPostulate{believe\KatlaUnderscore{}me}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{y}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{transport}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{y}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{y}\KatlaNewline{}
\IdrisFunction{transport}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisKeyword{interface}\KatlaSpace{}\IdrisType{ProofIrrelevant}\KatlaSpace{}\IdrisBound{ty}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{canonical}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{ty}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{proofIrrelevant}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{u}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{ty}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{canonical}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{u}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{ProofIrrelevant}\KatlaSpace{}\IdrisType{Void}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{canonical}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{impossible}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{proofIrrelevant}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{u}\KatlaSpace{}\IdrisKeyword{impossible}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{ProofIrrelevant}\KatlaSpace{}\IdrisType{Unit}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{canonical}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{proofIrrelevant}\KatlaSpace{}\IdrisData{()}\KatlaSpace{}\IdrisData{()}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{byIrrelevance}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{ProofIrrelevant}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\IdrisFunction{byIrrelevance}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{transport}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{proofIrrelevant}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{canonical}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{))}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{getSingleton}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\IdrisFunction{getSingleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*pure>
\begin{code}
\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSingleton}
\end{code}
%</pure>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*fmap>
\begin{code}
\IdrisFunction{(<\$>)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\IdrisBound{f}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</fmap>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*ap>
\begin{code}
\IdrisFunction{(<*>)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisFunction{<*>}\KatlaSpace{}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</ap>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Show}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisType{Show}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Cast}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisType{Cast}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{x}
\end{code}



==> Lib.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Lib}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Buffer}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Vect}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{failWith}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{String}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\IdrisFunction{failWith}\KatlaSpace{}\IdrisBound{str}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\IdrisKeyword{(}\IdrisPostulate{idris\KatlaUnderscore{}crash}\KatlaSpace{}\IdrisBound{str}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{etaUnit}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{()}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{()}\KatlaNewline{}
\IdrisFunction{etaUnit}\KatlaSpace{}\IdrisData{()}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}
\end{code}
<*toNat>
\begin{code}
\IdrisFunction{bits8AsBoundedNat}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bits8}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisType{**}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n}\KatlaSpace{}\IdrisFunction{<=}\KatlaSpace{}\IdrisData{255}\IdrisKeyword{)}\IdrisType{)}\KatlaNewline{}
\IdrisFunction{bits8AsBoundedNat}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}(\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisPostulate{believe\KatlaUnderscore{}me}\KatlaSpace{}\IdrisData{Oh})
\end{code}
</toNat>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*pair>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Tuple}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{(\#)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fst}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{snd}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{b}
\end{code}
%</pair>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*true>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{True}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{I}
\end{code}
%</true>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{export}
\end{code}
%<*etaTrue>
\begin{code}
\IdrisFunction{etaTrue}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{True}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\IdrisFunction{etaTrue}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}
\end{code}
%</etaTrue>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{curry}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Tuple}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\IdrisFunction{curry}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{y}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}
\end{code}
%<*etaTuple>
\begin{code}
\IdrisFunction{etaTuple}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Tuple}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fst}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{snd}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{etaTuple}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}
\end{code}
%</etaTuple>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{parameters}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Buffer}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setInts}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setInts}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setInts}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{is}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisFunction{setInt}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setInts}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{8}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{is}
\end{code}



==> Motivating.idr.tex <==

\begin{code}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}
\end{code}
%<*motivation>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Leaf}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Node}\KatlaSpace{}\IdrisType{Tree}\KatlaSpace{}\IdrisType{Bits8}\KatlaSpace{}\IdrisType{Tree}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{sum}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Leaf}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Node}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}
\end{code}
%</motivation>



==> SafeFolds.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{SafeFolds}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Lib}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Serialised.Desc}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{SaferIndexed}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Singleton}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%hide}\KatlaSpace{}Serialised.Desc.Data.fold\KatlaNewline{}
\IdrisKeyword{\%hide}\KatlaSpace{}SaferIndexed.Pointer.View.fold\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}

\end{code}
%<*datafold>
\begin{code}
\IdrisKeyword{parameters}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{alg}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Alg}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\IdrisKeyword{\{\})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{s}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{t}
\end{code}
%</datafold>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Pointer}\KatlaNewline{}

\end{code}
%<*pointerfold>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{parameters}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{alg}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Alg}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\IdrisKeyword{\{\})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{rec}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisBound{rec}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisFunction{>>=}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\IdrisKeyword{\{\})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{I}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{w}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{fmapFold}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{w}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{v}
\end{code}
%</pointerfold>
\begin{code}



==> SaferIndexed.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{SaferIndexed}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Fin}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.DPair}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Vect}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Buffer}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{System.File.Buffer}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Decidable.Equality}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.String}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Singleton}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Lib}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Serialised.Desc}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{blockSize}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\IdrisFunction{blockSize}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{1000}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Data}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{All'}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}

\end{code}
%<*allquant>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{All'}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}
\end{code}
%</allquant>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}

\end{code}
%<*dataallquant>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{All'}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{All'}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(\#)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{u}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{All'}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}
\end{code}
%</dataallquant>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{all}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{all}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{all}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{all}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{all}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{all}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{all}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fst}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{AllK}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{snd}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{curry}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{All}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{curry}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{etaTrue}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{I}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{curry}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{curry}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{f}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{SaferIndexed.Data.curry}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{snd}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{SaferIndexed.Data.curry}\KatlaSpace{}\IdrisBound{e}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{w}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{etaTuple}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{curry}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Serialising}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*serialising>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{MkSerialising}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{runSerialising}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Buffer}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{Int}
\end{code}
%</serialising>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*serialisingbind>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{(>>=)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisBound{io}\KatlaSpace{}\IdrisFunction{>>=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSerialising}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\IdrisBound{buf}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisBound{io}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{runSerialising}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}
\end{code}
%</serialisingbind>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{parameters}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Buffer}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{o}\KatlaSpace{}\IdrisType{Int,}\KatlaSpace{}\IdrisType{Int}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{layer}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{[],}\KatlaSpace{}\IdrisBound{start}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{layer}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{[],}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<\$}\KatlaSpace{}\IdrisFunction{setBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{getSingleton}\KatlaSpace{}\IdrisBound{layer}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n1}\IdrisData{,}\KatlaSpace{}\IdrisBound{afterLeft}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n2}\IdrisData{,}\KatlaSpace{}\IdrisBound{afterRight}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisBound{afterLeft}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{w}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n1}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{n2}\IdrisData{,}\KatlaSpace{}\IdrisBound{afterRight}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{layer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{end}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{runSerialising}\KatlaSpace{}\IdrisBound{layer}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{(}\IdrisData{,}\IdrisBound{end}\IdrisKeyword{)}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{if}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{then}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{else}\KatlaSpace{}\IdrisData{[}\IdrisBound{end}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisBound{start}\IdrisData{]}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMu}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{consNumber}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{c}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Constructor}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{c}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{c}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMu}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{cons}\KatlaSpace{}\IdrisBound{layer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}[\KatlaSpace{}Tag\KatlaSpace{}|\KatlaSpace{}...\KatlaSpace{}offsets\KatlaSpace{}...\KatlaSpace{}|\KatlaSpace{}...\KatlaSpace{}meaning\KatlaSpace{}...\KatlaSpace{}]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cast}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{to}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{afterTag}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{afterOffs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{afterTag}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{8}\KatlaSpace{}\IdrisFunction{*}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{offsets}\KatlaSpace{}\IdrisBound{cons}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{is}\IdrisData{,}\KatlaSpace{}\IdrisBound{end}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{goMeaning}\KatlaSpace{}\IdrisBound{afterOffs}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{cons}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{layer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setInts}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{afterTag}\KatlaSpace{}\IdrisBound{is}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{end}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*serialisemu>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{(\#)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{All}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</serialisemu>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisBound{layer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSerialising}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{buf}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{goMu}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{index}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{constructors}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{layer}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setMuK}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{AllK}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setMuK}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{index}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{constructors}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{cons}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{SaferIndexed.Data.curry}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{cons}\IdrisKeyword{)}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{layer}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{MkSerialising}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{buf}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{goMu}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{cons}\KatlaSpace{}\IdrisBound{layer}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{serialiseToFile}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{String}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{serialiseToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{newBuffer}\KatlaSpace{}\IdrisFunction{blockSize}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Nothing}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisData{"\textbackslash{}\{\KatlaUnderscore{}\KatlaUnderscore{}LOC\KatlaUnderscore{}\KatlaUnderscore{}\}\KatlaSpace{}Couldn't\KatlaSpace{}allocate\KatlaSpace{}buffer"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{end}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{setData}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{8}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setInt}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{end}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisData{8}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{size}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{runSerialising}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{end}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Right}\KatlaSpace{}\IdrisData{()}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{writeBufferToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{size}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Left}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{err}\IdrisData{,}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{err}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{()}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Buffer}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*serialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{serialise}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}
\end{code}
%</serialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{serialise}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{all}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\IdrisFunction{Buffer.serialise}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Compact}
\end{code}
%<*compactserialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{serialise}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}
\end{code}
%</compactserialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{serialise}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Buffer.serialise}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Pointer}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*elem>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{MkMeaning}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{subterms}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{o}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{meaningBuffer}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Buffer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{meaningPosition}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{meaningSize}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}
\end{code}
%</elem>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*pointermu>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{MkMu}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{muBuffer}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Buffer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{muPosition}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{muSize}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}
\end{code}
%</pointermu>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Poke}\KatlaNewline{}
\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Poke'}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*pokedatafun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Poke'}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}
\end{code}
%</pokedatafun>
\begin{code}

\end{code}
%<*pokedatadata>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Poke'}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Poke'}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(\#)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{u}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Poke'}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}
\end{code}
%</pokedatadata>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*pokefun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Poke}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</pokefun>
%<*pokefunNone>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{None}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{el}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{etaTrue}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{I}\IdrisKeyword{)}
\end{code}
%</pokefunNone>
%<*pokefunByte>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Byte}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{el}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getBits8}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{meaningBuffer}\KatlaSpace{}\IdrisBound{el}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{meaningPosition}\KatlaSpace{}\IdrisBound{el}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisPostulate{unsafeMkSingleton}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}
\end{code}
%</pokefunByte>
%<*pokefunProd>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Prod}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{sl}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ol}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{t}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkMeaning}\KatlaSpace{}\IdrisBound{sub}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisBound{size}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{subl}\IdrisData{,}\KatlaSpace{}\IdrisBound{subr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisBound{ol}\KatlaSpace{}\IdrisBound{sub}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{sizel}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{subl}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{sl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{left}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkMeaning}\KatlaSpace{}\IdrisBound{subl}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisBound{sizel}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{posr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{sizel}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{right}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkMeaning}\KatlaSpace{}\IdrisBound{subr}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{posr}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{size}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisBound{sizel}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{etaTuple}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{left}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{right}\IdrisKeyword{)}
\end{code}
%</pokefunProd>
%<*pokefunRec>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Rec}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkMeaning}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisBound{size}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkMu}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisBound{size}\IdrisKeyword{)}
\end{code}
%</pokefunRec>
%</pokefunbody>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Layer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Layer'}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*layerdata>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Layer}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Layer}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Layer}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Layer}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Layer'}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Layer'}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Layer'}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(\#)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Layer}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Layer}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{u}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Layer'}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}
\end{code}
%</layerdata>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*layerfun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Layer}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisBound{el}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{el}\KatlaSpace{}\IdrisFunction{>>=}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{s}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{.}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Layer}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{p}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{p}
\end{code}
%</layerfun>
\begin{code}

\end{code}
%<*layerexample>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{example}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisData{Byte}\IdrisKeyword{))}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{example}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisFunction{>>=}\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{q}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}?hole
\end{code}
%</layerexample>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*outdata>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Out}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(\#)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Out}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</outdata>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*getIndex>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getIndex}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getIndex}\KatlaSpace{}\IdrisBound{mu}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{tag}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getBits8}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{muBuffer}\KatlaSpace{}\IdrisBound{mu}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{muPosition}\KatlaSpace{}\IdrisBound{mu}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{natToFin}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{tag}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{consNumber}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisData{"Invalid\KatlaSpace{}representation"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}
\end{code}
%</getIndex>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*outfun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Out}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</outfun>
%<*outfunbody>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{t}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{mu}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getIndex}\KatlaSpace{}\IdrisBound{mu}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{sub}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisPostulate{unfoldAs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{val}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisFunction{getConstructor}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{sub}\IdrisFunction{.fst}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\IdrisBound{sub}\IdrisFunction{.snd}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{mu}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisBound{sub}\IdrisFunction{.snd}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{val}\IdrisKeyword{)}
\end{code}
%</outfunbody>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}

\end{code}
%<*getOffsets>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getOffsets}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Buffer}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{pos}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getOffsets}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisBound{pos}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getOffsets}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{off}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getInt}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getOffsets}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{8}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{pos}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{off}\KatlaSpace{}\IdrisData{::}\IdrisKeyword{))}
\end{code}
%</getOffsets>
\begin{code}
\KatlaNewline{}

\end{code}
%<*getConstructor>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getConstructor}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getConstructor}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{mu}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisFunction{offs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat};\KatlaSpace{}\IdrisFunction{offs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{offsets}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{index}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{constructors}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getOffsets}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{muBuffer}\KatlaSpace{}\IdrisBound{mu}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{1}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisFunction{muPosition}\KatlaSpace{}\IdrisBound{mu}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{offs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{size}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{muSize}\KatlaSpace{}\IdrisBound{mu}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{8}\KatlaSpace{}\IdrisFunction{*}\KatlaSpace{}\IdrisFunction{offs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{subterms}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{MkMeaning}\KatlaSpace{}\IdrisBound{subterms}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{muBuffer}\KatlaSpace{}\IdrisBound{mu}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisBound{size}
\end{code}
%</getConstructor>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Pure}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaNewline{}

\end{code}
%<*pureisleaf>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isLeaf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bool}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isLeaf}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isLeaf}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{False}
\end{code}
%</pureisleaf>
%<*isleaf>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isLeaf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isLeaf}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isLeaf}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisFunction{>>=}\KatlaSpace{}\IdrisKeyword{\textbackslash{}case}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisKeyword{|]}
\end{code}
%</isleaf>
\begin{code}
\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{View}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*viewdata>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(\#)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisFunction{Layer}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</viewdata>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{PRINTONLY}\KatlaNewline{}

\end{code}
%<*view>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{View}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{el}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{vs}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisBound{el}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{vs}\IdrisKeyword{)}
\end{code}
%</view>
\begin{code}
\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*viewfun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{View}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</viewfun>
%<*viewfunbody>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{el}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{vs}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisBound{el}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{vs}\IdrisKeyword{)}
\end{code}
%</viewfunbody>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*fmaptype>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)))}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.fmap}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}
\end{code}
%</fmaptype>
%<*fmapfun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisFunction{>>=}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\IdrisKeyword{\{\})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.fmap}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{fv}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{fw}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{w}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisBound{fv}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{fw}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{v}
\end{code}
%</fmapfun>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Monad}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\IdrisKeyword{\{\})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)))}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.traverse}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisFunction{>>=}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\IdrisKeyword{\{\})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisFunction{Poke}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.traverse}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{I}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{w}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{w}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{(\#)}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<*>}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisFunction{<*>}\KatlaSpace{}\IdrisBound{w}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}

\end{code}
%<*foldtype>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{alg}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Alg}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.fold}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}
\end{code}
%</foldtype>

%<*foldfun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{rec}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmap}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{alg}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisBound{rec}\IdrisKeyword{)}
\end{code}
%</foldfun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*deserialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{deserialise}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</deserialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{deserialise}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmap}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{id}\KatlaSpace{}\IdrisFunction{deserialise}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisFunction{transport}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{id}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Refl}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Compact}
\end{code}
%<*compactdeserialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{deserialise}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</compactdeserialise>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{deserialise}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{View.deserialise}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Serialising}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*copy>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{copy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{copy}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSerialising}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{buf}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{size}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{muSize}\KatlaSpace{}\IdrisBound{ptr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{copyData}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{muBuffer}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{muPosition}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{size}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{pos}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{size}\IdrisKeyword{)}
\end{code}
%</copy>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Tree}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Find\KatlaSpace{}a\KatlaSpace{}byte}
\end{code}
%<*tfindB>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{findB}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bits8}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bool}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{findB}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{False}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisFunction{||}\KatlaSpace{}\IdrisFunction{findB}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{||}\KatlaSpace{}\IdrisFunction{findB}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{r}
\end{code}
%</tfindB>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*path>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Path}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bits8}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Here}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Path}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{TurnL}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Path}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Path}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{TurnR}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Path}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Path}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}
\end{code}
%</path>
\begin{code}

\end{code}
%<*tfind>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{find}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{tgt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bits8}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Maybe}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Path}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{find}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Nothing}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisData{No}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{decEq}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Yes}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{Here}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{TurnL}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisFunction{find}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{<|>}\KatlaSpace{}\IdrisData{TurnR}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisFunction{find}\KatlaSpace{}\IdrisBound{tgt}\KatlaSpace{}\IdrisBound{r}
\end{code}
%</tfind>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Tree\KatlaSpace{}sum}
\end{code}
%<*tsum>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Z}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}
\end{code}
%</tsum>
\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Raw}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Raw\KatlaSpace{}sum}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*rsum>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{Z}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}
\end{code}
%</rsum>
\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Lazy}
\end{code}
%<*pokerightmost>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Maybe}\KatlaSpace{}\IdrisType{Bits8}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{Nothing}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{el}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{br}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{el}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{br}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{mval}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{mval}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{mval}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Nothing}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Just}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{getSingleton}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{))}
\end{code}
%</pokerightmost>

\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Strict}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*viewrightmost>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Maybe}\KatlaSpace{}\IdrisType{Bits8}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{Nothing}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{mval}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{mval}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{mval}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Nothing}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Just}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{getSingleton}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{))}
\end{code}
%</viewrightmost>
\begin{code}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Here\KatlaSpace{}we\KatlaSpace{}define\KatlaSpace{}the\KatlaSpace{}functional\KatlaSpace{}specification\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}functions\KatlaSpace{}we}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}want\KatlaSpace{}to\KatlaSpace{}write\KatlaSpace{}over\KatlaSpace{}pointers.\KatlaSpace{}This\KatlaSpace{}will,\KatlaSpace{}via\KatlaSpace{}Singleton\KatlaSpace{}\&\KatlaSpace{}Serialising,}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}allow\KatlaSpace{}us\KatlaSpace{}to\KatlaSpace{}write\KatlaSpace{}correct\KatlaSpace{}by\KatlaSpace{}construction\KatlaSpace{}effectful\KatlaSpace{}functions}\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Data}\KatlaNewline{}

\end{code}
%<*rightmost>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Maybe}\KatlaSpace{}\IdrisType{Bits8}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Nothing}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{mval}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{rightmost}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fromMaybe}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{mval}\IdrisKeyword{)}
\end{code}
%</rightmost>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}The\KatlaSpace{}size\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}tree\KatlaSpace{}is\KatlaSpace{}given\KatlaSpace{}by\KatlaSpace{}the\KatlaSpace{}number\KatlaSpace{}of\KatlaSpace{}nodes}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{size}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{size}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{l}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}The\KatlaSpace{}sum\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}tree's\KatlaSpace{}node\KatlaSpace{}is\KatlaSpace{}given\KatlaSpace{}by\KatlaSpace{}casting\KatlaSpace{}the\KatlaSpace{}Bits8\KatlaSpace{}nodes}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}to\KatlaSpace{}Nat\KatlaSpace{}and\KatlaSpace{}summing\KatlaSpace{}them\KatlaSpace{}up}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Map\KatlaSpace{}is\KatlaSpace{}obtained\KatlaSpace{}by\KatlaSpace{}applying\KatlaSpace{}a\KatlaSpace{}function\KatlaSpace{}transforming\KatlaSpace{}Bit8\KatlaSpace{}values}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}to\KatlaSpace{}all\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}Bits8\KatlaSpace{}stored\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}tree's\KatlaSpace{}nodes}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Bits8}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bits8}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{leaf}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisFunction{node}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Here\KatlaSpace{}we\KatlaSpace{}define\KatlaSpace{}the\KatlaSpace{}effectful\KatlaSpace{}functions\KatlaSpace{}processing\KatlaSpace{}a\KatlaSpace{}pointer}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}IO\KatlaSpace{}allows\KatlaSpace{}us\KatlaSpace{}to\KatlaSpace{}inspect\KatlaSpace{}the\KatlaSpace{}content\KatlaSpace{}addressed\KatlaSpace{}by\KatlaSpace{}the\KatlaSpace{}pointer\KatlaSpace{}to\KatlaSpace{}take\KatlaSpace{}the\KatlaSpace{}tree\KatlaSpace{}apart}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Serialising\KatlaSpace{}lets\KatlaSpace{}us\KatlaSpace{}build\KatlaSpace{}a\KatlaSpace{}specified\KatlaSpace{}output\KatlaSpace{}tree}\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Pointer}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Correct\KatlaSpace{}by\KatlaSpace{}construction\KatlaSpace{}size\KatlaSpace{}function.}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}t\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}phantom\KatlaSpace{}name\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}tree\KatlaSpace{}represented\KatlaSpace{}by\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}ptr\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}position\KatlaSpace{}of\KatlaSpace{}t\KatlaSpace{}inside\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}Singleton\KatlaSpace{}ensures\KatlaSpace{}that\KatlaSpace{}the\KatlaSpace{}value\KatlaSpace{}we\KatlaSpace{}return\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}same\KatlaSpace{}as\KatlaSpace{}if}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}we\KatlaSpace{}had\KatlaSpace{}directly\KatlaSpace{}processed\KatlaSpace{}`t`.}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{size}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.size}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{size}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkSingleton}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{br}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{size}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{l}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{br}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{size}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{poke}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{|]}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Correct\KatlaSpace{}by\KatlaSpace{}construction\KatlaSpace{}sum\KatlaSpace{}function.}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}t\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}phantom\KatlaSpace{}name\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}tree\KatlaSpace{}represented\KatlaSpace{}by\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}ptr\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}position\KatlaSpace{}of\KatlaSpace{}t\KatlaSpace{}inside\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}Singleton\KatlaSpace{}ensures\KatlaSpace{}that\KatlaSpace{}the\KatlaSpace{}value\KatlaSpace{}we\KatlaSpace{}return\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}same\KatlaSpace{}as\KatlaSpace{}if}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}we\KatlaSpace{}had\KatlaSpace{}directly\KatlaSpace{}processed\KatlaSpace{}`t`.}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*csum>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Singleton}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.sum}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{sum}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{|]}\KatlaSpace{}\IdrisKeyword{|]}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{|]}
\end{code}
%</csum>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisFunction{Tree.leaf}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{setMuK}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{node}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Singleton}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Tree.node}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{node}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{setMuK}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{PRINTONLY}
\end{code}
%<*serialisedmapcompact>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bits8}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bits8}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{r}
\end{code}
%</serialisedmapcompact>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Correct\KatlaSpace{}by\KatlaSpace{}construction\KatlaSpace{}map\KatlaSpace{}function.}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}f\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}function\KatlaSpace{}to\KatlaSpace{}map\KatlaSpace{}over\KatlaSpace{}the\KatlaSpace{}tree's\KatlaSpace{}nodes}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}t\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}phantom\KatlaSpace{}name\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}tree\KatlaSpace{}represented\KatlaSpace{}by\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}ptr\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}position\KatlaSpace{}of\KatlaSpace{}t\KatlaSpace{}inside\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}Serialising\KatlaSpace{}ensures\KatlaSpace{}that\KatlaSpace{}the\KatlaSpace{}value\KatlaSpace{}we\KatlaSpace{}compute\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}same\KatlaSpace{}as\KatlaSpace{}if}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}we\KatlaSpace{}had\KatlaSpace{}directly\KatlaSpace{}processed\KatlaSpace{}`t`.}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*serialisedmap>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bits8}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bits8}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{|]}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{r}
\end{code}
%</serialisedmap>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Simple\KatlaSpace{}printing\KatlaSpace{}function}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{display}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{String}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{display}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{out}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{layer}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{display}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{display}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{"(node\KatlaSpace{}\textbackslash{}\{}\IdrisBound{l}\IdrisData{\}\KatlaSpace{}\textbackslash{}\{}\IdrisFunction{show}\IdrisData{\KatlaSpace{}}\IdrisKeyword{(}\IdrisFunction{getSingleton}\IdrisData{\KatlaSpace{}}\IdrisBound{b}\IdrisKeyword{)}\IdrisData{\}\KatlaSpace{}\textbackslash{}\{}\IdrisBound{r}\IdrisData{\})"}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Serialising}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*execSerialising>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{execSerialising}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</execSerialising>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{execSerialising}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{newBuffer}\KatlaSpace{}\IdrisFunction{blockSize}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Nothing}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisData{"\textbackslash{}\{\KatlaUnderscore{}\KatlaUnderscore{}LOC\KatlaUnderscore{}\KatlaUnderscore{}\}\KatlaSpace{}Couldn't\KatlaSpace{}allocate\KatlaSpace{}buffer"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{middle}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{setData}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{8}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setInt}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{middle}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisData{8}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{end}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{runSerialising}\KatlaSpace{}\IdrisBound{act}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{middle}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkMu}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{middle}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{end}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisBound{middle}\IdrisKeyword{))}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{FilePath}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\IdrisFunction{FilePath}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{String}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}readFromFile\KatlaSpace{}creates\KatlaSpace{}a\KatlaSpace{}pointer\KatlaSpace{}to\KatlaSpace{}a\KatlaSpace{}datastructure\KatlaSpace{}stored\KatlaSpace{}in\KatlaSpace{}a\KatlaSpace{}file}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}@\KatlaSpace{}cs\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}datatype\KatlaSpace{}you\KatlaSpace{}want\KatlaSpace{}to\KatlaSpace{}use\KatlaSpace{}to\KatlaSpace{}decode\KatlaSpace{}the\KatlaSpace{}buffer's\KatlaSpace{}content}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}@\KatlaSpace{}safe\KatlaSpace{}signals\KatlaSpace{}whether\KatlaSpace{}to\KatlaSpace{}check\KatlaSpace{}the\KatlaSpace{}file's\KatlaSpace{}header\KatlaSpace{}matches\KatlaSpace{}the\KatlaSpace{}declared\KatlaSpace{}datatype}
\end{code}
%<*readFromFile>
\begin{code}
\IdrisFunction{readFromFile}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{default}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{safe}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{FilePath}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Exists}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{))}\KatlaNewline{}
\IdrisFunction{readFromFile}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{fp}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisData{Right}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{createBufferFromFile}\KatlaSpace{}\IdrisBound{fp}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Left}\KatlaSpace{}\IdrisBound{err}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{err}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{skip}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getInt}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{when}\KatlaSpace{}\IdrisBound{safe}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{cs'}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getData}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{8}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{unless}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{eqData}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{cs'}\IdrisKeyword{)}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{unlines}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{[}\KatlaSpace{}\IdrisData{"Description\KatlaSpace{}mismatch:"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{,}\KatlaSpace{}\IdrisData{"expected:",}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{cs}\IdrisData{,}\KatlaSpace{}\IdrisData{"but\KatlaSpace{}got:",}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{cs'}\KatlaSpace{}\IdrisData{]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{skip}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{8}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Evidence}\KatlaSpace{}\IdrisFunction{t}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkMu}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisKeyword{(!(}\IdrisFunction{rawSize}\KatlaSpace{}\IdrisBound{buf}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{\KatlaDash{}}\KatlaSpace{}\IdrisBound{pos}\IdrisKeyword{)))}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{where}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisFunction{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}postulated\KatlaSpace{}as\KatlaSpace{}an\KatlaSpace{}abstract\KatlaSpace{}value}
\end{code}
%</readFromFile>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Pointer}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*writeToFile>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{FilePath}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkMu}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisBound{size}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{desc}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getInt}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{8}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{desc}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{bufSize}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{8}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{desc}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{size}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisKeyword{if}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{then}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{else}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisBound{newbuf}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{newBuffer}\KatlaSpace{}\IdrisBound{bufSize}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Nothing}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisData{"\textbackslash{}\{\KatlaUnderscore{}\KatlaUnderscore{}LOC\KatlaUnderscore{}\KatlaUnderscore{}\}\KatlaSpace{}Couldn't\KatlaSpace{}allocate\KatlaSpace{}buffer"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{copyData}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisBound{newbuf}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{copyData}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{pos}\KatlaSpace{}\IdrisBound{size}\KatlaSpace{}\IdrisBound{newbuf}\KatlaSpace{}\IdrisBound{start}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{buf}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Right}\KatlaSpace{}\IdrisData{()}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{writeBufferToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{bufSize}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Left}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{err}\IdrisData{,}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{err}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{()}
\end{code}
%</writeToFile>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Serialising}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{String}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{forall}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{.}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisBound{val}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{execSerialising}\KatlaSpace{}\IdrisBound{val}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Data}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{String}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisBound{fp}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{serialise}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Data}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{swap}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{swap}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisData{I}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{swap}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Pointer}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*swap>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{swap}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Serialising}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Data.swap}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{swap}\KatlaSpace{}\IdrisBound{ptr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ptr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisData{I}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisData{I}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisFunction{\#}\KatlaSpace{}\IdrisFunction{copy}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{copy}\KatlaSpace{}\IdrisBound{l}
\end{code}
%</swap>
\begin{code}
\KatlaNewline{}
\IdrisFunction{testing}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Pointer.Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\IdrisFunction{testing}\KatlaSpace{}\IdrisBound{tree}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{putStrLn}\KatlaSpace{}\IdrisData{"Tree:\KatlaSpace{}\textbackslash{}\{}\IdrisKeyword{!(}\IdrisFunction{display}\IdrisData{\KatlaSpace{}}\IdrisBound{tree}\IdrisKeyword{)}\IdrisData{\}"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{putStrLn}\KatlaSpace{}\IdrisData{"RSum:\KatlaSpace{}\textbackslash{}\{}\IdrisFunction{show}\IdrisData{\KatlaSpace{}}\IdrisKeyword{!(}\IdrisFunction{Raw.sum}\IdrisData{\KatlaSpace{}}\IdrisBound{tree}\IdrisKeyword{)}\IdrisData{\}"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{putStrLn}\KatlaSpace{}\IdrisData{"Sum:\KatlaSpace{}\textbackslash{}\{}\IdrisFunction{show}\IdrisData{\KatlaSpace{}}\IdrisKeyword{!(}\IdrisFunction{Pointer.sum}\IdrisData{\KatlaSpace{}}\IdrisBound{tree}\IdrisKeyword{)}\IdrisData{\}"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{putStrLn}\KatlaSpace{}\IdrisData{"Rightmost:\KatlaSpace{}\textbackslash{}\{}\IdrisFunction{show}\IdrisData{\KatlaSpace{}}\IdrisKeyword{!(}\IdrisFunction{rightmost}\IdrisData{\KatlaSpace{}}\IdrisBound{tree}\IdrisKeyword{)}\IdrisData{\}"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{putStrLn}\KatlaSpace{}\IdrisData{"Tree\KatlaSpace{}size:\KatlaSpace{}\textbackslash{}\{}\IdrisFunction{show}\IdrisData{\KatlaSpace{}}\IdrisKeyword{!(}\IdrisFunction{size}\IdrisData{\KatlaSpace{}}\IdrisBound{tree}\IdrisKeyword{)}\IdrisData{\}"}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{main}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{()}\KatlaNewline{}
\IdrisFunction{main}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}First\KatlaSpace{}Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{writeToFile}\KatlaSpace{}\IdrisData{"tmp"}\KatlaSpace{}\IdrisFunction{example}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisBound{tree}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{readFromFile}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisData{"tmp"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testing}\KatlaSpace{}\IdrisBound{tree}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{putStrLn}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{replicate}\KatlaSpace{}\IdrisData{72}\KatlaSpace{}\IdrisData{'\KatlaDash{}'}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Second\KatlaSpace{}Tree:\KatlaSpace{}mapping\KatlaSpace{}over\KatlaSpace{}the\KatlaSpace{}first\KatlaSpace{}one}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{serialiseToFile}\KatlaSpace{}\IdrisData{"tmp2"}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{1}\IdrisFunction{+}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{tree}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisBound{tree2}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{readFromFile}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisData{"tmp2"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testing}\KatlaSpace{}\IdrisBound{tree2}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{putStrLn}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{replicate}\KatlaSpace{}\IdrisData{72}\KatlaSpace{}\IdrisData{'\KatlaDash{}'}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Third\KatlaSpace{}Tree:\KatlaSpace{}don't\KatlaSpace{}go\KatlaSpace{}via\KatlaSpace{}a\KatlaSpace{}file}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisBound{tree3}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{execSerialising}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{2}\IdrisFunction{+}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{tree2}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testing}\KatlaSpace{}\IdrisBound{tree3}
\end{code}



==> Serialised/Desc.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Serialised.Desc}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Buffer}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Fin}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.String}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Vect}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Decidable.Equality}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Lib}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Types}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}description\KatlaSpace{}is\KatlaSpace{}a\KatlaSpace{}nested\KatlaSpace{}tuple\KatlaSpace{}of\KatlaSpace{}Bytes\KatlaSpace{}or\KatlaSpace{}recursive\KatlaSpace{}positions}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}It\KatlaSpace{}is\KatlaSpace{}indexed\KatlaSpace{}by\KatlaSpace{}1\KatlaSpace{}'input'\KatlaSpace{}parameter\KatlaSpace{}and\KatlaSpace{}2\KatlaSpace{}'ouput'\KatlaSpace{}indices:}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}\KatlaSpace{}@rightmost\KatlaSpace{}telling\KatlaSpace{}us\KatlaSpace{}whether\KatlaSpace{}we\KatlaSpace{}are\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}rightmost\KatlaSpace{}subterm}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}in\KatlaSpace{}which\KatlaSpace{}case\KatlaSpace{}`Rec`\KatlaSpace{}won't\KatlaSpace{}need\KatlaSpace{}to\KatlaSpace{}record\KatlaSpace{}an\KatlaSpace{}additional\KatlaSpace{}offset}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}\KatlaSpace{}@static\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}the\KatlaSpace{}statically\KatlaSpace{}known\KatlaSpace{}part\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}size\KatlaSpace{}(in\KatlaSpace{}number\KatlaSpace{}of\KatlaSpace{}bytes)}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}\KatlaSpace{}@offsets\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}the\KatlaSpace{}dynamically\KatlaSpace{}known\KatlaSpace{}part\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}size\KatlaSpace{}(in\KatlaSpace{}number\KatlaSpace{}of\KatlaSpace{}subtrees)}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*desctype>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{rightmost}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{static}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{offsets}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Type}
\end{code}
%</desctype>
%<*desc>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Prod}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{sl}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sr}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ol}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{or}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{sl}\KatlaSpace{}\IdrisBound{ol}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{sr}\KatlaSpace{}\IdrisBound{or}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sl}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{sr}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ol}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{or}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{ifThenElse}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}
\end{code}
%</desc>
\begin{code}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}constructor\KatlaSpace{}description\KatlaSpace{}is\KatlaSpace{}essentially\KatlaSpace{}an\KatlaSpace{}existential\KatlaSpace{}type}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}around\KatlaSpace{}a\KatlaSpace{}description}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}@\KatlaSpace{}nm\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}type\KatlaSpace{}of\KatlaSpace{}name\KatlaSpace{}we\KatlaSpace{}use\KatlaSpace{}for\KatlaSpace{}the\KatlaSpace{}constructor}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*constructor>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Constructor}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{nm}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{(::)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{name}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{nm}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisFunction{static}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisFunction{offsets}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{description}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{static}\KatlaSpace{}\IdrisBound{offsets}
\end{code}
%</constructor>
\begin{code}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}data\KatlaSpace{}description\KatlaSpace{}is\KatlaSpace{}a\KatlaSpace{}sum\KatlaSpace{}over\KatlaSpace{}a\KatlaSpace{}list\KatlaSpace{}of\KatlaSpace{}constructor\KatlaSpace{}types}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*data>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{nm}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{MkData}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisFunction{consNumber}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{auto}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisFunction{fitsInBits8}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{consNumber}\IdrisFunction{\KatlaSpace{}<=\KatlaSpace{}255}\IdrisKeyword{)\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{constructors}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{consNumber}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Constructor}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}
\end{code}
%</data>
\begin{code}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}wrapper\KatlaSpace{}around\KatlaSpace{}fin\KatlaSpace{}that\KatlaSpace{}helps\KatlaSpace{}unification}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*index>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{MkIndex}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getIndex}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{consNumber}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}
\end{code}
%</index>
\begin{code}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}smart\KatlaSpace{}projection}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*description>
\begin{code}
\IdrisFunction{description}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{cons}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{index}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{getIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{constructors}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{static}\KatlaSpace{}\IdrisBound{cons}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{offsets}\KatlaSpace{}\IdrisBound{cons}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{description}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{description}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{index}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{getIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{constructors}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{))}
\end{code}
%</description>
\begin{code}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}little\KatlaSpace{}bit\KatlaSpace{}of\KatlaSpace{}magic}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{isConstructor}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Eq}\KatlaSpace{}\IdrisBound{nm}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisBound{nm}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Maybe}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{cs}\IdrisFunction{.consNumber}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{isConstructor}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{findIndex}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{==}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisFunction{Constructor.name}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{constructors}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*fromString>
\begin{code}
\IdrisFunction{fromString}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisType{String}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{str}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{String}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{auto}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{IsJust}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isConstructor}\KatlaSpace{}\IdrisBound{str}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\IdrisFunction{fromString}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{str}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isConstructor}\KatlaSpace{}\IdrisBound{str}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}
\end{code}
%</fromString>
\begin{code}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Another\KatlaSpace{}kind\KatlaSpace{}of\KatlaSpace{}magic}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{fromInteger}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nm}\IdrisKeyword{\}\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{auto}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{consNumber}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{/=}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\IdrisFunction{fromInteger}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkData}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\IdrisData{::}\IdrisKeyword{\KatlaUnderscore{})\}}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkIndex}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{restrict}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{DecEq}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{decEq}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{l}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{decEq}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{l}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{decEq}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisKeyword{.(}\IdrisBound{k}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Yes}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Yes}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{decEq}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIndex}\KatlaSpace{}\IdrisBound{l}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{No}\KatlaSpace{}\IdrisBound{notEq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{No}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisBound{notEq}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{getIndex}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{))}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Show\KatlaSpace{}instances}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Show}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{showPrec}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"\KatlaUnderscore{}"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{showPrec}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Bits8"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{showPrec}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{showParens}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Open}\KatlaSpace{}\IdrisFunction{<}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{"Tuple\KatlaSpace{}\textbackslash{}\{}\IdrisFunction{showPrec}\IdrisData{\KatlaSpace{}App\KatlaSpace{}}\IdrisBound{d}\IdrisData{\}\KatlaSpace{}\textbackslash{}\{}\IdrisFunction{showPrec}\IdrisData{\KatlaSpace{}App\KatlaSpace{}}\IdrisBound{e}\IdrisData{\}"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{showPrec}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"X"}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Show}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nm}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{constructors}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Constructor}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{String}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"⊥"}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{c}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{concat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{"μX.\KatlaSpace{}"}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{c}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{((}\IdrisData{"\KatlaSpace{}+\KatlaSpace{}"}\KatlaSpace{}\IdrisFunction{++}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{c}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{c}\IdrisKeyword{))}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Eq\KatlaSpace{}instances}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Heterogeneous\KatlaSpace{}equality\KatlaSpace{}check\KatlaSpace{}for\KatlaSpace{}descriptions}\KatlaNewline{}
\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r'}\KatlaSpace{}\IdrisBound{s'}\KatlaSpace{}\IdrisBound{n'}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bool}\KatlaNewline{}
\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisFunction{\&\&}\KatlaSpace{}\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{False}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{eqConstructor}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Constructor}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Constructor}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bool}\KatlaNewline{}
\IdrisFunction{eqConstructor}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{d}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqDesc}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Heterogeneous\KatlaSpace{}equality\KatlaSpace{}check\KatlaSpace{}for\KatlaSpace{}vectors\KatlaSpace{}of\KatlaSpace{}constructors}\KatlaNewline{}
\IdrisFunction{eqConstructors}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Constructor}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Constructor}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bool}\KatlaNewline{}
\IdrisFunction{eqConstructors}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\IdrisFunction{eqConstructors}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{c}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{c'}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{cs'}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqConstructor}\KatlaSpace{}\IdrisBound{c}\KatlaSpace{}\IdrisBound{c'}\KatlaSpace{}\IdrisFunction{\&\&}\KatlaSpace{}\IdrisFunction{eqConstructors}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{cs'}\KatlaNewline{}
\IdrisFunction{eqConstructors}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{False}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{eqData}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bool}\KatlaNewline{}
\IdrisFunction{eqData}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkData}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkData}\KatlaSpace{}\IdrisBound{cs'}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqConstructors}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{cs'}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Serialisation\KatlaSpace{}of\KatlaSpace{}descriptions\KatlaSpace{}to\KatlaSpace{}a\KatlaSpace{}Buffer}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{parameters}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{buf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Buffer}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Set\KatlaSpace{}a\KatlaSpace{}description\KatlaSpace{}in\KatlaSpace{}a\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}start\KatlaSpace{}position\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}buffer\KatlaSpace{}to\KatlaSpace{}set\KatlaSpace{}the\KatlaSpace{}description\KatlaSpace{}at}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}d\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}description\KatlaSpace{}to\KatlaSpace{}serialise}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}Returns\KatlaSpace{}the\KatlaSpace{}end\KatlaSpace{}position}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<\$}\KatlaSpace{}\IdrisFunction{setBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<\$}\KatlaSpace{}\IdrisFunction{setBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisFunction{setBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{2}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{afterLeft}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{d}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisBound{afterLeft}\KatlaSpace{}\IdrisBound{e}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{<\$}\KatlaSpace{}\IdrisFunction{setBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{3}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Set\KatlaSpace{}a\KatlaSpace{}list\KatlaSpace{}of\KatlaSpace{}constructors\KatlaSpace{}one\KatlaSpace{}after\KatlaSpace{}the\KatlaSpace{}other\KatlaSpace{}in\KatlaSpace{}a\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}start\KatlaSpace{}position\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}buffer\KatlaSpace{}to\KatlaSpace{}set\KatlaSpace{}the\KatlaSpace{}constructors\KatlaSpace{}at}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}cs\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}list\KatlaSpace{}of\KatlaSpace{}constructors\KatlaSpace{}to\KatlaSpace{}serialise}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}Returns\KatlaSpace{}the\KatlaSpace{}end\KatlaSpace{}position}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setConstructors}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Constructor}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}))}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setConstructors}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{start}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setConstructors}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{((\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{d}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisBound{afterC}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{setDesc}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisBound{d}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setConstructors}\KatlaSpace{}\IdrisBound{afterC}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Set\KatlaSpace{}data\KatlaSpace{}description\KatlaSpace{}in\KatlaSpace{}a\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}start\KatlaSpace{}position\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}buffer\KatlaSpace{}to\KatlaSpace{}set\KatlaSpace{}the\KatlaSpace{}data\KatlaSpace{}description\KatlaSpace{}at}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}cs\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}data\KatlaSpace{}description\KatlaSpace{}to\KatlaSpace{}serialise}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}Returns\KatlaSpace{}the\KatlaSpace{}end\KatlaSpace{}position}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setData}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisType{Int}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setData}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkData}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{consNumber}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}We\KatlaSpace{}first\KatlaSpace{}store\KatlaSpace{}the\KatlaSpace{}length\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}list\KatlaSpace{}so\KatlaSpace{}that\KatlaSpace{}we\KatlaSpace{}know\KatlaSpace{}how}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}many\KatlaSpace{}constructors\KatlaSpace{}to\KatlaSpace{}deserialise\KatlaSpace{}on\KatlaSpace{}the\KatlaSpace{}way\KatlaSpace{}out}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{consNumber}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{setConstructors}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Existential\KatlaSpace{}wrapper\KatlaSpace{}to\KatlaSpace{}deserialise\KatlaSpace{}descriptions}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}rightmost\KatlaSpace{}is\KatlaSpace{}known\KatlaSpace{}statically\KatlaSpace{}but\KatlaSpace{}the\KatlaSpace{}others\KatlaSpace{}indices\KatlaSpace{}are\KatlaSpace{}not}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{record}\KatlaSpace{}\IdrisType{IDesc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{rightmost}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{constructor}\KatlaSpace{}\IdrisData{MkIDesc}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisFunction{static}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisFunction{offsets}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{runIDesc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{rightmost}\KatlaSpace{}\IdrisBound{static}\KatlaSpace{}\IdrisBound{offsets}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Auxiliary\KatlaSpace{}definition\KatlaSpace{}to\KatlaSpace{}help\KatlaSpace{}idris\KatlaSpace{}figure\KatlaSpace{}out\KatlaSpace{}the\KatlaSpace{}types\KatlaSpace{}of}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}everything\KatlaSpace{}involved}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{IProd}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{IDesc}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IDesc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IDesc}\KatlaSpace{}\IdrisBound{r}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{IProd}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIDesc}\KatlaSpace{}\IdrisBound{d}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkIDesc}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkIDesc}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Get\KatlaSpace{}a\KatlaSpace{}description\KatlaSpace{}from\KatlaSpace{}a\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}start\KatlaSpace{}position\KatlaSpace{}the\KatlaSpace{}description\KatlaSpace{}starts\KatlaSpace{}at\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}Returns\KatlaSpace{}the\KatlaSpace{}end\KatlaSpace{}position\KatlaSpace{}\&\KatlaSpace{}the\KatlaSpace{}description}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getDesc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Int,}\KatlaSpace{}\IdrisType{IDesc}\KatlaSpace{}\IdrisBound{r}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getDesc}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisKeyword{!(}\IdrisFunction{getBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1,}\KatlaSpace{}\IdrisData{MkIDesc}\KatlaSpace{}\IdrisData{None}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1,}\KatlaSpace{}\IdrisData{MkIDesc}\KatlaSpace{}\IdrisData{Byte}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{2}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{afterLeft}\IdrisData{,}\KatlaSpace{}\IdrisBound{d}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{getDesc}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{False}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{end}\IdrisData{,}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{getDesc}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{r}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{afterLeft}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{end}\IdrisData{,}\KatlaSpace{}\IdrisFunction{IProd}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{3}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1,}\KatlaSpace{}\IdrisData{MkIDesc}\KatlaSpace{}\IdrisData{Rec}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{failWith}\KatlaSpace{}\IdrisData{"Invalid\KatlaSpace{}Description"}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Get\KatlaSpace{}a\KatlaSpace{}list\KatlaSpace{}of\KatlaSpace{}constructor\KatlaSpace{}from\KatlaSpace{}a\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}start\KatlaSpace{}position\KatlaSpace{}the\KatlaSpace{}list\KatlaSpace{}of\KatlaSpace{}constructors\KatlaSpace{}starts\KatlaSpace{}at\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}n\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}number\KatlaSpace{}of\KatlaSpace{}constructors\KatlaSpace{}to\KatlaSpace{}deserialise}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getConstructors}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Constructor}\KatlaSpace{}\IdrisType{()}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getConstructors}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisData{[]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getConstructors}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{afterD}\IdrisData{,}\KatlaSpace{}\IdrisBound{d}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getDesc}\KatlaSpace{}\IdrisBound{start}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getConstructors}\KatlaSpace{}\IdrisBound{afterD}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisKeyword{((}\IdrisData{()}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisFunction{runIDesc}\KatlaSpace{}\IdrisBound{d}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Get\KatlaSpace{}a\KatlaSpace{}data\KatlaSpace{}description\KatlaSpace{}from\KatlaSpace{}a\KatlaSpace{}buffer}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}start\KatlaSpace{}position\KatlaSpace{}the\KatlaSpace{}data\KatlaSpace{}description\KatlaSpace{}starts\KatlaSpace{}at\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}buffer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getData}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Int}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{IO}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nm}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{()}\IdrisKeyword{\})}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{getData}\KatlaSpace{}\IdrisBound{start}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{do}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{<\KatlaDash{}}\KatlaSpace{}\IdrisFunction{getBits8}\KatlaSpace{}\IdrisBound{buf}\KatlaSpace{}\IdrisBound{start}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}(\IdrisBound{n}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisBound{oh})\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{bits8AsBoundedNat}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{MkData}\KatlaSpace{}\IdrisFunction{<\$>}\KatlaSpace{}\IdrisFunction{getConstructors}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{start}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Meaning\KatlaSpace{}of\KatlaSpace{}descriptions\KatlaSpace{}as\KatlaSpace{}functors}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Data}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Meaning\KatlaSpace{}where\KatlaSpace{}subterms\KatlaSpace{}are\KatlaSpace{}interpreted\KatlaSpace{}using\KatlaSpace{}the\KatlaSpace{}parameter}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*meaningtype>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}
\end{code}
%</meaningtype>
%<*meaningfun>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{True}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Bits8}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Tuple}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{x}
\end{code}
%</meaningfun>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*fmap>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmap}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}
\end{code}
%</fmap>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{t}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong2}\KatlaSpace{}\IdrisData{(\#)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisBound{u}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fmapId}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisBound{t}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*traverse>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Monad}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{d}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Desc}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisBound{s}\KatlaSpace{}\IdrisBound{o}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisData{None}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pure}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{e}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{w}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{[|}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisBound{d}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisBound{e}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{w}\KatlaSpace{}\IdrisKeyword{|]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{traverse}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{v}
\end{code}
%</traverse>
\begin{code}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Meaning\KatlaSpace{}of\KatlaSpace{}data\KatlaSpace{}descriptions\KatlaSpace{}as\KatlaSpace{}fixpoints}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*alg>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Alg}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Alg}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{x}
\end{code}
%</alg>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Fixpoint\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}description:}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}1.\KatlaSpace{}pick\KatlaSpace{}a\KatlaSpace{}constructor}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}2.\KatlaSpace{}give\KatlaSpace{}its\KatlaSpace{}meaning\KatlaSpace{}where\KatlaSpace{}subterms\KatlaSpace{}are\KatlaSpace{}entire\KatlaSpace{}subtrees}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*mu>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(\#)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Alg}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{))}
\end{code}
%</mu>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*unfoldAs>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\%unsafe}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisFunction{unfoldAs}\KatlaSpace{}\IdrisKeyword{:}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{(}\IdrisBound{val}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Data.Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Data.Mu}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{**}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{val}\IdrisKeyword{)}\IdrisType{)}
\end{code}
%</unfoldAs>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Fixpoints\KatlaSpace{}are\KatlaSpace{}initial\KatlaSpace{}algebras}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*fold>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisBound{nm}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisFunction{Alg}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{alg}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{(}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{fmap}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fold}\KatlaSpace{}\IdrisBound{alg}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{t}\IdrisKeyword{)}
\end{code}
%</fold>
\begin{code}
\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}\KatlaDash{}}\KatlaNewline{}
\IdrisComment{\KatlaDash{}\KatlaDash{}\KatlaSpace{}Examples}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Tree}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*treeleaf>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Leaf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Constructor}\KatlaSpace{}\IdrisType{String}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Leaf}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisData{None}
\end{code}
%</treeleaf>
%<*treeleafmeaning>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{MeaningLeaf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisFunction{Leaf}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisType{True}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{MeaningLeaf}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}
\end{code}
%</treeleafmeaning>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*treenode>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Node}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Constructor}\KatlaSpace{}\IdrisType{String}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Node}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisData{Prod}\KatlaSpace{}\IdrisData{Rec}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Prod}\KatlaSpace{}\IdrisData{Byte}\KatlaSpace{}\IdrisData{Rec}\IdrisKeyword{)}
\end{code}
%</treenode>
%<*treenodemeaning>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{MeaningNode}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{Meaning}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{description}\KatlaSpace{}\IdrisFunction{Node}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisType{Tuple}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Tuple}\KatlaSpace{}\IdrisType{Bits8}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{MeaningNode}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}
\end{code}
%</treenodemeaning>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*treedesc>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Data}\KatlaSpace{}\IdrisType{String}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkData}\KatlaSpace{}\IdrisData{[}\IdrisFunction{Leaf}\IdrisData{,}\KatlaSpace{}\IdrisFunction{Node}\IdrisData{]}
\end{code}
%</treedesc>

\end{code}
%<*indexleaf>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{indexLeaf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{indexLeaf}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Leaf"}
\end{code}
%</indexleaf>

\end{code}
%<*notindexcons>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{failing}\KatlaSpace{}\IdrisFunction{notIndexCons}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Index}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{notIndexCons}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Cons"}
\end{code}
%</notindexcons>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*leaf>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Leaf"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisData{I}
\end{code}
%</leaf>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*node>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{node}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Bits8}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{node}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{r}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{"Node"}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{l}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisData{\#}\KatlaSpace{}\IdrisBound{r}
\end{code}
%</node>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{TYPESETTINGONLY}
\end{code}
%<*longexample>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{example}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{example}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{leaf}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{5}\KatlaSpace{}\IdrisFunction{leaf}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{10}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisData{20}\KatlaSpace{}\IdrisFunction{leaf}\IdrisKeyword{))}
\end{code}
%</longexample>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}
\end{code}
%<*example>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{example}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Mu}\KatlaSpace{}\IdrisFunction{Tree}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{example}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{node}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{leaf}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{5}\KatlaSpace{}\IdrisFunction{leaf}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{10}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{node}\KatlaSpace{}\IdrisFunction{leaf}\KatlaSpace{}\IdrisData{20}\KatlaSpace{}\IdrisFunction{leaf}\IdrisKeyword{)}
\end{code}
%</example>



==> Snoc.idr.tex <==

\begin{code}
\KatlaNewline{}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Snoc}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}

\end{code}
%<*Snoc>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Snoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Lin}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Snoc}\KatlaSpace{}\IdrisData{[]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{(:<)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{init}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{last}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Snoc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{init}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisData{[}\IdrisBound{last}\IdrisData{]}\IdrisKeyword{)}
\end{code}
%</Snoc>
\begin{code}

\end{code}
%<*unsnoc>
\begin{code}
\IdrisFunction{unsnoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Snoc}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\IdrisFunction{unsnoc}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\IdrisFunction{unsnoc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{unsnoc}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{init}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{last}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{init}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{last}
\end{code}
%</unsnoc>



==> With.idr.tex <==

\begin{code}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{partial}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{e}\IdrisKeyword{,}\KatlaSpace{}\IdrisFunction{rhs1}\IdrisKeyword{,}\KatlaSpace{}\IdrisFunction{rhs2}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\IdrisFunction{e}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{3}\KatlaNewline{}
\IdrisFunction{rhs1}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\IdrisFunction{rhs2}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{SUGAR}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}
\end{code}
%<*fsugar>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{f}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{e}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{rhs1}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{rhs2}
\end{code}
%</fsugar>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{DESUGAR}\KatlaNewline{}
\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{f}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fAux}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{\KatlaDash{}>}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}

\end{code}
%<*fdesugar>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fAux}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{rhs1}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fAux}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{rhs2}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{f}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{fAux}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisFunction{e}
\end{code}
%</fdesugar>
\begin{code}
\KatlaNewline{}

\end{code}



==> hoare.tex <==
\section{Analogy to Separation Logic}\label{appendix:hoare}

Some readers may feel uneasy about the fact that parts of our
library are implemented using \idris{} escape hatches.
%
This section justifies this practice by drawing an analogy to
separation logic~\citep{DBLP:journals/cacm/OHearn19,DBLP:books/hal/Chargueraud23,MANUAL:book/sfoundations/Chargueraud23}
and highlighting that this practice corresponds
to giving an axiomatisation of the runtime behaviour of our
library's core functions.

\newcommand{\Pointer}[3]{\ensuremath{#1 \xmapsto{#2} #3}}
\newcommand{\Hoare}[4]{\ensuremath{\lbrace~ #1 ~\rbrace~ #2 ~\lbrace~ #3.\, #4 ~\rbrace}}
\newcommand{\Meaning}[2]{\ensuremath{\llbracket \,#1\, \rrbracket\, (\Mu{#2})}}
\newcommand{\Mu}[1]{\ensuremath{\mu \, \mathit{#1}}}

\subsection{Interlude: Separation Logic}

A Hoare triple~\citep{DBLP:journals/cacm/Hoare69} of the form
\[ \Hoare{P}{e}{v}{Q} \]
states that under the precondition
$P$, and binding the result of evaluating the expression $e$ as $v$,
we can prove that $Q$ holds.
%
One of the basic predicates of separation logic~\citep{DBLP:conf/lics/Reynolds02}
is a `points to' assertion (\Pointer{\ell}{}{t}) stating that
the label $\ell$ points to a memory location containing $t$.

A separation logic proof system then typically consists in defining
a language and providing axioms characterising the behaviour of
each language construct.
%
The simplest example involving memory is perhaps a language
with pointers to bytes and a single \texttt{deref} construct
dereferencing a pointer.
%
We can then give the following axiom
\[ \Hoare{\Pointer{\ell}{}{\mathit{bs}}}{\texttt{deref}\,\ell}{v}{\mathit{bs} = v \ast \Pointer{\ell}{}{\mathit{bs}}} \]
to characterise \texttt{deref} by stating that the value
it returns is precisely the one the pointer is referencing,
and that the pointer is still valid and still referencing
the same value after it has been dereferenced.

The axioms can be combined to prove statements about more
complex programs such as the following silly one for instance.
Here we state that if we dereference the pointer a first time,
discard the result and then dereference it once more then we
end up in the same situation as if we had dereferenced it only once.
\[ \Hoare{\Pointer{\ell}{}{\mathit{bs}}}{\texttt{deref}\,\ell;\, \texttt{deref}\,\ell}{v}{\mathit{bs} = v \ast \Pointer{\ell}{}{\mathit{bs}}} \]

Note that in all of these rules $\mathit{bs}$ is only present
in the specification layer. \texttt{deref} itself cannot possibly
return $\mathit{bs}$ directly, it needs to actually perform an
effectful operation that will read the memory cell's content.

\subsection{Characterising Our Library}

We are going to explain that we can see our library as a small
embedded Domain Specific
Language (eDSL)~\citep{DBLP:journals/csur/Hudak96}
that has \IdrisFunction{poke} and \IdrisFunction{out} as
sole language constructs.
%
Our main departure from separation logic is that we want to
program in a correct-by-construction fashion and so the types
of \IdrisFunction{poke} and \IdrisFunction{out} have to be
just as informative as the axioms we would postulate
in separation logic.
%
This dual status of the basic building blocks being both
executable programs \emph{and} an axiomatic specification
of their respective behaviour is precisely why their
implementations in \idris{} necessarily uses unsafe features.

Our pointers are not simply referring to raw memory locations
that contain unstructured words, they come with a strong invariant
about the underlying data that is stored.
In that sense, they are closer to representation
predicates~\citep{MANUAL:book/sfoundations/Chargueraud23}.

Our pointers are not just referring to memory locations containing
words but rather typed
pointers to complex data structures.

We are going to write \Pointer{\ell}{\Meaning{d}{cs}}{t} for the assumption
that we own a pointer $\ell$ of type
(\IdrisType{Pointer.Meaning} \IdrisBound{d} \IdrisBound{cs} \IdrisBound{t}),
and \Pointer{\ell}{\Mu{cs}}{t} for the assumption that we own
a pointer $\ell$ of type (\IdrisType{Pointer.Mu} \IdrisBound{cs} \IdrisBound{t}).
%
In case we do not care about the type of the pointer at hand
(e.g. because it can be easily inferred from the context), we
will simply write \Pointer{\ell}{}{t}.


\subsubsection{Axioms for poke}\label{sec:axiom-poke}

Thinking in terms of Hoare triples, if we have a pointer
$\ell$ to a term $t$ known to be a single byte then
(\IdrisFunction{poke} $\ell$)
will return a byte $bs$ and allow us to observe that $t$ is
equal to that byte.
\[
\Hoare
    {\Pointer{\ell}{\Meaning{\text{\IdrisData{Byte}}}{cs}}{t}}
    {\text{\IdrisFunction{poke}}\,\ell}
    {\mathit{bs}}
    {t = \mathit{bs} \ast \ell \mapsto t}
\]
Similarly, if the pointer $\ell$ is for a pair then
(\IdrisFunction{poke} $\ell$) will
reveal that the term $t$ can be taken apart into the pairing
of two terms $t_1$ and $t_2$ and
return a pointer for each of these components.
\begin{gather*}
\Hoare
    {\Pointer{\ell}{\Meaning{\text{\IdrisData{Prod}}\, d_1 d_2}{cs}}{t}}
    {\\\text{\IdrisFunction{poke}}\,\ell\\}
    {(\ell_1,\, \ell_2)}
    {\exists t_1.\, \exists t_2.\, t = (t_1 \,\text{\IdrisData{\#}}\, t_2)
        \ast \ell \mapsto t \ast \Pointer{\ell_1}{\Meaning{d_1}{cs}}{t_1} \ast \Pointer{\ell_2}{\Meaning{d_2}{cs}}{t_2}}
\end{gather*}
Last but not least, poking a pointer with the \IdrisData{Rec}
description will return another pointer for the same value but
at a different type.
\[
\Hoare
    {\Pointer{\ell}{\Meaning{\text{\IdrisData{Rec}}}{cs}}{t}}
    {\text{\IdrisFunction{poke}}\,\ell}
    {\ell_1}
    {\Pointer{\ell_1}{\Mu{cs}}{t} \ast \Pointer{\ell}{}{t}}
\]

\subsubsection{Example of a Derived Rule for layer}

Given that \IdrisFunction{layer} is defined in terms of \IdrisFunction{poke},
we do not need to postulate any axioms to characterise it and can instead
prove lemmas.
%
We will skip the proofs here but give an example of a derived rule.
%
Using the description (\IdrisData{Prod} \IdrisData{Rec} (\IdrisData{Prod} \IdrisData{Byte} \IdrisData{Rec}))
of the arguments to a node in our running example of binary trees,
\IdrisFunction{layer}'s behaviour would be characterised by the following
statement.
\begin{gather*}
\Hoare
    {\Pointer{\ell}{\Meaning{\text{\IdrisData{Prod} \IdrisData{Rec} (\IdrisData{Prod} \IdrisData{Byte} \IdrisData{Rec})}}{cs}}{t}}
    {\\\text{\IdrisFunction{layer}}\,\ell\\}
    {(\ell_1,\, bs,\, \ell_2)}
    {\exists t_1.\, \exists t_2.\,
      t = (t_1 \,\text{\IdrisData{\#}}\, bs \,\text{\IdrisData{\#}}\, t_2)
      \ast \Pointer{\ell_1}{\Mu{cs}}{t_1}
      \ast \Pointer{\ell_2}{\Mu{cs}}{t_2}
      \ast \Pointer{\ell}{}{t}}
\end{gather*}
It states that provided a pointer to such a meaning,
calling \IdrisFunction{layer} would
return a triple of
a pointer $\ell_1$ for the left subtree,
the byte $\mathit{bs}$ stored in the node,
and a pointer $\ell_2$ for the right subtree.

\subsubsection{Axiom for out}

The only other construct for our small DSL is the function \IdrisFunction{out}.
Things are a lot simpler here as the return type
is not defined by induction on the description.
As a consequence we only need the following axiom.
\[
\Hoare
    {\Pointer{\ell}{\Mu{cs}}{t}}
    {\text{\IdrisFunction{out}}\,\ell}
    {(k,\, \ell_1)}
    {\exists t_1.\, t = (k \,\text{\IdrisData{\#}}\, t_1)
      \ast \Pointer{\ell}{}{t} \ast \Pointer{\ell_1}{\Meaning{cs_k}{cs}}{t_1}}
\]
It states that under the condition that $\ell$ points to $t$,
(\IdrisFunction{out} $\ell$) returns a pair of an index
and a pointer to the meaning of the description associated to that index by $cs$,
and allows us to learn that $t$ is constructed using that index
and that meaning.

By combining \IdrisFunction{out} and \IdrisFunction{layer} we could once
more define a derived rule and prove e.g. that every tree can be taken
apart as either a leaf or a node with a pointer to a left subtree, a byte,
and a pointer to a right subtree i.e. what \IdrisFunction{view} does in
our library.


==> robust-catch.tex <==
\makeatletter

\newrobustcmd*\OrigExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\global\expandafter\CatchFBT@tok\expandafter{%
\expandafter}\the\CatchFBT@tok
}%\OrigExecuteMetaData

\newrobustcmd*\ChkExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\edef\mytokens{\detokenize\expandafter{\the\CatchFBT@tok}}
\ifx\mytokens\empty\PackageError{catchfilebetweentags}{the tag #2 is not found\MessageBreak in file #1 \MessageBreak called from \jobname.tex}{use a different tag}\fi%
}%\ChkExecuteMetaData

\renewrobustcmd*\ExecuteMetaData[2][\jobname]{%
\ChkExecuteMetaData[#1]{#2}%
\OrigExecuteMetaData[#1]{#2}%
}

\makeatother

